The Strongest 100 Point Radio Sources in the LMC at 1.4 GHz

We present the 100 strongest 1.4 GHz point sources from a new mosaic image in the direction of the Large Magellanic Cloud (LMC). The observations making up the mosaic were made over a ten year period and were combined with Parkes single dish data at 1.4 GHz to complete the image for short spacing. An initial list of co-identifications within 10" at 0.843, 4.8 and 8.6 GHz consisted of 2682 sources. Elimination of extended objects and artifact noise allowed the creation of a refined list containing 1988 point sources. Most of these are presumed to be background objects seen through the LMC; a small portion may represent compact H II regions, young SNRs and radio planetary nebulae. For the 1988 point sources we find a preliminary average spectral index of -0.53 and present a 1.4 GHz image showing source location in the direction of the LMC.

==> BULL-ZAG.TEX <==
\magnification=\magstep0
\baselineskip=3.1truemm 
\vsize=230truemm 
\hsize=165truemm 
\parindent=1truecm
\parskip=0pt plus2truept 

\def\nav{\leavevmode\lower.5em\hbox{"}} 

\def\hang{\hangindent\parindent}
\def\item{\par\hang\textindent}
\def\itemitem{\par\indent \hangindent2\parindent \textindent}
\def\textindent#1{\indent\llap{#1\enspace}\ignorespaces}

\catcode`@=11

\newdimen\pagewidth \newdimen\pageheight \newdimen\ruleht
  \maxdepth=2.2pt  \parindent=.5truecm
\pagewidth=\hsize  \pageheight=\vsize  \ruleht=.5pt
\abovedisplayskip=6pt plus 3pt minus 1pt
\belowdisplayskip=6pt plus 3pt minus 1pt
\abovedisplayshortskip=0pt plus 3pt 
\belowdisplayshortskip=4pt plus 3pt 

\newinsert\margin
\dimen\margin=\maxdimen
\count\margin=0 \skip\margin=0pt

\def\footnote#1{\edef\@sf{\spacefactor\the\spacefactor}#1\@sf
     \insert\footins\bgroup\eightrm
     \insertlinepenalty100 \let\par=\endgraf
       \leftskip=0pt \rightskip=0pt
       \splittopskip=10pt plus 1pt minus 1pt \floatingpenalty20000
       \smallskip\item{#1}\bgroup\strut\aftergroup\@foot\let\next}
\skip\footins=12pt plus 2pt minus 4pt
\dimen\footins=.6truecm
\newif\iftitle
\def\titlepage{\global\titletrue}

\def\headl{\vbox to 1cm{{\ifodd\pageno\rightheadline \else 
\leftheadline\fi}\vskip1mm\hrule}} 
\def\headr{\vbox to 1cm{}}
\headline={\ifnum\pageno=\ppp \vbox{\headr} \else \vbox{\headl} \fi}  

\def\rightheadline{\hbox to \pagewidth{\centerline{\rhead}}} 
\def\leftheadline{\hbox to \pagewidth{\centerline{\lhead}}}

\def\makefootline{\baselineskip=2truecc \line{\the\footline}}
  \def\nonumbers{\hbox to \pagewidth{
                 \vbox to 6mm{}
                 \hfill}}
\footline{\ifodd\pageno\rightfootline
          \else\leftfootline\fi}
  \def\rightfootline{\hbox to \pagewidth{
                     \vbox to 6mm{}
                     \hfill\tenrm\folio}}
  \def\leftfootline{\hbox to \pagewidth{
                     \vbox to 6mm{}
                     \tenrm\kern-8pt\folio\hfill}}

\def\onepageout#1{\shipout\vbox{
  \offinterlineskip
\vbox to 1cm{\ifnum\pageno=\ppp \vbox{\headr} \else 
\vbox{\headl} \fi}
  \vbox to \pageheight{
    \ifvoid\margin\else
     \rlap{\kern31cc\vbox to0pt{\kern4pt\box\margin \vss}}\fi
    #1
    \ifvoid\footins\else
     \vskip\skip\footins \kern-3pt
     \hrule height\ruleht width 4cm \kern-\ruleht \kern3pt
     \unvbox\footins\fi
    \boxmaxdepth=\maxdepth}
  \vbox to \pageheight{
     \ifnum\pageno<500     
     {\ifodd\pageno\rightfootline\else\leftfootline\fi} 
     \else\nonumbers\fi}}
\advancepageno}
               
\def\setcornerrules{\hbox to \pagewidth{
    \vrule width 1cc height\ruleht \hfil \vrule width 1cc}
  \hbox to \pagewidth{\llap{\sevenrm(page \folio)\kern1cc}
    \vrule height1cc width\ruleht depth0pt
    \hfil \vrule width\ruleht depth0pt}}
\output{\onepageout{\unvbox255}}
 
\newbox\partialpage

\def\dvekolone{\begingroup
  \output={\global\setbox\partialpage=\vbox{\unvbox255}}\eject
  \output={\doublecolumnout} \hsize=80mm \vsize=460mm}
 
\def\krajdvekolone{\output={\balancecolumns}\eject
  \endgroup \pagegoal=\vsize}

\def\doublecolumnout{\splittopskip=\topskip \splitmaxdepth=\maxdepth
  \dimen@=230mm \advance\dimen@ by-\ht\partialpage
  \setbox0=\vsplit255 to\dimen@ \setbox2=\vsplit255 to\dimen@
  \onepageout\pagesofar \unvbox255 \penalty\outputpenalty}

\def\pagesofar{\unvbox\partialpage
  \wd0=\hsize \wd2=\hsize \hbox to\pagewidth{\box0\hfil\box2}}

\def\balancecolumns{\setbox0=\vbox{\unvbox255} \dimen@=\ht0
  \advance\dimen@ by\topskip \advance\dimen@ by-\baselineskip
  \divide\dimen@ by2 \splittopskip=\topskip
  {\vbadness=10000 \loop \global\setbox3=\copy0
    \global\setbox1=\vsplit3 to\dimen@
    \ifdim\ht3>\dimen@ \global\advance\dimen@ by1pt \repeat}
  \setbox0=\vbox to\dimen@{\unvbox1} \setbox2=\vbox to\dimen@{\unvbox3}
  \pagesofar}

\def\cstok#1{\leavevmode\thinspace\hbox{\vrule\vtop{\vbox{\hrule\kern3pt
             \hbox{\vphantom\thinspace{#1}\thinspace}}
             \kern3pt\hrule}\vrule}\thinspace}    

\def\okvir#1{\vbox{\hrule\hbox{\vrule\kern0mm
             \vbox{\kern3mm#1\kern3mm}\kern0mm\vrule}\hrule}}

\def\boxit#1{\vbox{\hrule\hbox{\vrule\kern1mm
             \vbox{\kern1mm#1\kern1mm}\kern1mm\vrule}\hrule}}


\def\leftdisplay#1$${\leftline{\indent$\displaystyle{#1}$}$$}

\def\br{\break}%

\voffset=-.3cm
%\hoffset=.3cm
\hoffset=-.2cm






==> astro.tex <==
\def\tg{\mathop{\rm tg}\nolimits}
\def\arctg{\mathop{\rm arctg}\nolimits}

\def\point#1{\hbox{\setbox7=\hbox to0.8em{\hfil.\hfil}%
\setbox8=\hbox to0.8em{\hfil$^{#1}$\hfil}%
\box7\kern-0.8em\box8}}

\def\dd{\point{\rm d}}
\def\hh{\point{\rm h}}
\def\mm{\point{\rm m}}
\def\ss{\point{\rm s}}

\def\oo{\point{\circ}}
\def\ll{\point{\prime}}
\def\uu{\point{\prime\prime}}




==> mjyu.tex <==
\def\nava{\leavevmode\hbox{,\kern-0.09em,}}%yu-navodnik-pocetni
\def\navb{\char'134}                                      %yu-navodnik-krajnji
\def\DJ{\leavevmode\setbox0=\hbox{D}\kern0pt
 \rlap{\kern.04em\raise.188\ht0\hbox{-}}D}
\def\dj{\leavevmode\setbox0=\hbox{d}\kern0pt
 \rlap{\kern.215em\raise.46\ht0\hbox{-}}d}
\def\SH{\v S} \def\sh{\v s} % Sasinci
\def\CJ{\' C} \def\cj{\' c} % Cicevac
\def\CH{\v C} \def\ch{\v c} % Xaxak
\def\Z{\v Z} \def\z{\v z} % Zuzemberk
\def\br{\break}



==> wncyr.tex <==
\def\rrmd{\font\tipo=wncyr12\tip}%
\def\rbfd{\font\tipo=wncyb12\tip}%
\def\rssd{\font\tipo=wncyss12\tip}%
\def\rrm{\font\tipo=wncyr10\tip}%
\def\rbf{\font\tipo=wncyb10\tip}%
\def\rit{\font\tipo=wncyi10\tip}%
\def\rss{\font\tipo=wncyss10\tip}%
\def\rsc{\font\tipo=wncysc10\tip}%
\def\rrmdev{\font\tipo=wncyr9\tip}%
\def\rbfdev{\font\tipo=wncyb9\tip}%
\def\ritdev{\font\tipo=wncyi9\tip}%
\def\rssdev{\font\tipo=wncyss9\tip}%
\def\rrmos{\font\tipo=wncyr8\tip}%
\def\rbfos{\font\tipo=wncyb8\tip}%
\def\ritos{\font\tipo=wncyi8\tip}%
\def\rssos{\font\tipo=wncyss8\tip}%
\def\rrmsev{\font\tipo=wncyr7\tip}%
\def\rbfsev{\font\tipo=wncyb7\tip}%
\def\ritsev{\font\tipo=wncyi7\tip}%
\def\tip{\relax\tipo\def\DD{\tipo\char'006}\def\dd{\tipo\char'016}% \tip
\def\DJ{\DD}\def\dj{\dd}% 
\def\ZZ{\tipo\char'021}\def\zz{\tipo\char'031}%
\def\Z{\ZZ}\def\z{\zz}%
\def\LJ{\tipo\char'001}\def\lj{\tipo\char'011}%
\def\NJ{\tipo\char'000}\def\nj{\tipo\char'010}%
\def\CC{\tipo\char'007}\def\cc{\tipo\char'017}%
\def\DZ{\tipo\char'002}\def\dz{\tipo\char'012}%
\def\XX{Q}\def\xx{q}%
\def\JJ{J}\def\jj{j}% 
\def\SS{X}\def\ss{x}%
\def\JA{\tipo\char'027}\def\ja{\tipo\char'037}%
\def\SC{W}\def\sc{w}%
\def\CJ{\CC}\def\cj{\cc}%
\def\CH{Q}\def\ch{q}%
\def\SH{X}\def\sh{x}%
% sch="x"; tvrdo i = "y"; ja = "j"; schtsch = "w"; tsch = "q"
\def\EE{\tipo\char'003}\def\ee{\tipo\char'013}% "e oborotnoe"
\def\JI{\tipo\char'022}\def\ji{\tipo\char'032}% rusko "j"
\def\JU{\tipo\char'020}\def\ju{\tipo\char'030}%
\def\M{\tipo\char'136}\def\m{\tipo\char'176}% meki znak
\def\TV{\tipo\char'137}\def\tv{\tipo\char'177}% tvrdi znak
\def\rnava{\tipo\char'074}\def\rnavb{\tipo\char'076}% ruski navodnici
\def\snava{\leavevmode\hbox{,\kern-0.06em,}}% yu-
\def\snavb{\tipo\char'134}}% navodnici
\def\br{\break}%



